Collaborative OLAP with Tag Clouds: Web 2.0 OLAP Formalism and Experimental Evaluation

Increasingly, business projects are ephemeral. New Business Intelligence tools must support ad-lib data sources and quick perusal. Meanwhile, tag clouds are a popular community-driven visualization technique. Hence, we investigate tag-cloud views with support for OLAP operations such as roll-ups, slices, dices, clustering, and drill-downs. As a case study, we implemented an application where users can upload data and immediately navigate through its ad hoc dimensions. To support social networking, views can be easily shared and embedded in other Web sites. Algorithmically, our tag-cloud views are approximate range top-k queries over spontaneous data cubes. We present experimental evidence that iceberg cuboids provide adequate online approximations. We benchmark several browser-oblivious tag-cloud layout optimizations.

==> abstract.tex <==
\fontsize{9}{11}\selectfont
Increasingly, business projects are ephemeral. 
New Business Intelligence tools must support ad-lib data sources and
quick perusal.
Meanwhile, tag clouds are a popular community-driven visualization technique. 
Hence, we investigate tag-cloud views with support
for OLAP operations such as roll-ups, slices, dices, clustering, and drill-downs. As a case study, we
implemented an application where users can upload  data 
and immediately navigate through its ad hoc dimensions. 
To support social networking, views can be easily shared 
and embedded in other Web sites. 
Algorithmically, our tag-cloud views are approximate range top-k queries
over spontaneous data cubes. We present experimental evidence that 
iceberg cuboids provide adequate online approximations. 
We benchmark several browser-oblivious tag-cloud layout optimizations.

==> authors.tex <==
\author{{\textmd {\textbf }}\\
  \fontsize{11}{13}\selectfont
  Kamel Aouiche, Daniel Lemire and Robert Godin\\
  \fontsize{9}{11}\selectfont
  \textit{Universit\'e du Qu\'ebec \`a Montr\'eal, 100 Sherbrooke West, Montreal, Canada}\\
  \fontsize{9}{11}\selectfont
  \textit{kamel.aouiche@gmail.com, lemire@acm.org, godin.robert@uqam.ca}\\[12pt]
  %
  % repeat previous group of commands here for further authors
}


==> keywords.tex <==
\fontsize{9}{11}\selectfont OLAP, Data Warehouse, Business Intelligence, Tag
Cloud, Social Web
%The paper should have at least one keyword. The text should be set in 9-point
%font size and without the use of bold or italic font style.


==> title.tex <==
% The Title is all in Uppercase
\newcommand{\mytitle}{\uppercase{Collaborative OLAP with Tag Clouds}\\
% The Subtitle should have initial letters capitalized
\fontsize{13}{15}\selectfont \textit{Web 2.0 OLAP Formalism and Experimental Evaluation}
}


